A Collaborative Approach Using Neural Networks for BLE-RSS Lateration-Based Indoor Positioning

In daily life, mobile and wearable devices with high computing power, together with anchors deployed in indoor environments, form a common solution for the increasing demands for indoor location-based services. Within the technologies and methods currently in use for indoor localization, the approaches that rely on Bluetooth Low Energy (BLE) anchors, Received Signal Strength (RSS), and lateration are among the most popular, mainly because of their cheap and easy deployment and accessible infrastructure by a variety of devices. Nevertheless, such BLE- and RSS-based indoor positioning systems are prone to inaccuracies, mostly due to signal fluctuations, poor quantity of anchors deployed in the environment, and/or inappropriate anchor distributions, as well as mobile device hardware variability. In this paper, we address these issues by using a collaborative indoor positioning approach, which exploits neighboring devices as additional anchors in an extended positioning network. The collaborating devices' information (i.e., estimated positions and BLE-RSS) is processed using a multilayer perceptron (MLP) neural network by taking into account the device specificity in order to estimate the relative distances. After this, the lateration is applied to collaboratively estimate the device position. Finally, the stand-alone and collaborative position estimates are combined, providing the final position estimate for each device. The experimental results demonstrate that the proposed collaborative approach outperforms the stand-alone lateration method in terms of positioning accuracy.

==> Algorithm/Algo.tex <==
\begin{algorithm}[!htb]
 \caption{Estimation of collaborative device position}
 \label{alg:one}
 \begin{algorithmic}[1]
 \small
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 %\REQUIRE RSS values, $\eta$=$2.1$,  $RSSat1m$=\SI{-63.7816}{\dbm}, $threshold=\SI{-83}{\dbm}$
  \REQUIRE windows time: $wt=5s$
  \REQUIRE Deployed beacons information collected within a $wt$ (RSSI values and GT)
  \REQUIRE Collaborative devices information collected within a $wt$ (RSSI values, $\mathbf{\hat{P}_{dev}}$ and $\mathbf{\hat{\hat{P}}_{dev}}$ )
  \REQUIRE LDPL: $\eta = 2.1$ 
  \REQUIRE $RSSat1m$ (e.g., \SI{-63.7816}{\dbm} for device 2)
  %\REQUIRE $RSSat1m = [\SI{-63.7816}{\dbm},\SI{-63.9243}{\dbm},\SI{-72.7770}{\dbm},\SI{-63.54}{\dbm},\SI{-67}{\dbm}]$
  \REQUIRE $threshold = \SI{-83}{\dbm}$
  %\ENSURE $\mathbf{\hat{d}_{dev}}=[\hat{d}_{dev1},...\hat{d}_{dev4}]$
  
  \ENSURE Estimated position   $\hat{P}_{dev}$, $\hat{\hat{P}}_{dev}$ and $\mathbf{\hat{\hat{\hat{P}}}_{dev}}$ 

%\ENSURE  estimated position $\mathbf{\hat{\hat{P}}_{dev}}=[\hat{\hat{P}}_{dev1},...,\hat{\hat{P}}_{dev5}]$
%\ENSURE estimated position $\mathbf{\hat{\hat{\hat{P}}}_{dev}}=[\hat{\hat{\hat{P}}}_{dev1},...\hat{\hat{\hat{P}}}_{dev5}]$
\STATE Group the RSS values by beacon and device %(same minor \& major ID's)
\STATE Remove RSS outliers of each group
 \STATE Average RSS values of each group: $\overline{RSSI_{bcon}}(i)$ and $\overline{RSSI_{dev}}(i)$
   \FOR {$i\leftarrow$ 1 \textbf{to} number of $\overline{RSSI_{bcon}}(i)$}%$b_{AverageRSS}$}
 \IF {($\overline{RSSI_{bcon}}(i) \ge treshold $)}
  \STATE Include $i$-th beacon to reference beacons set ($ref_{BLEset}$)
  \ENDIF
  \ENDFOR
  \IF {(length($ref_{BLEset}$) $\ge 5 $)}
  \STATE Sort $ref_{BLEset}$ according to the corresponding RSSI values in descending order and remove those beacons above the 4\textsuperscript{th} position (e.g., 5\textsuperscript{th}, 6\textsuperscript{th}, $\ldots$)
  \ENDIF
  %%% No collaborative part
  %___________d\_hat\_bcon Function
  
  \STATE \textbf{Function} d\_hat\_bcon($ref_{BLEset}$, $\eta$, $RSSat1m$)
  \STATE Estimate the four relative distance between beacons of $ref_{BLEset}$ and the collaborative device position using Eq.\ref{eqn:pathloss}%, with values $\eta$ and $RSSat1m$
  \RETURN $\mathbf{\hat{d}_{bcon}}=[\hat{d}_{bcon1},...,\hat{d}_{bcon4}]$
  \STATE \textbf{end Function}
  %___________P\_hat\_dev Function
  \STATE \textbf{Function} P\_hat\_dev($\mathbf{\hat{d}_{bcon}}$, GT)
  \STATE Estimate the device position using the Levenberg-Marquardt Least Squares (L-MLS) Lateration method%, with values $\mathbf{\hat{d}_{bcon}}$ and GT 
  \RETURN $\hat{P}_{dev}$ (e.g., $\hat{P}_{dev2}$ for device 2)
  \STATE \textbf{end Function}

  \STATE \textbf{ Share the estimated device position ($\hat{P}_{dev}$)}
 %%% Collaborative part
   %___________d\_hat\_dev Function
  \STATE \textbf{Function} d\_hat\_dev($\overline{RSSI_{dev}}(i)$)
  \STATE Estimate the relative distance between near collaborative devices using the trained NN model%, with the $\overline{RSSI_{dev}}(i)$
  \RETURN $\mathbf{\hat{d}_{dev}}=[\hat{d}_{dev1},...\hat{d}_{dev4}]$
  \STATE \textbf{end Function}

  \STATE \textbf{Load devices position ($\mathbf{\hat{P}_{dev}}$)}
  %\STATE \textbf{ Share the estimated device distance ($\mathbf{\hat{d}_{dev}}$)}
  %___________P\_hat\_hat\_dev Function
  \STATE \textbf{Function} P\_hat\_hat\_dev($\mathbf{\hat{d}_{dev}}$,$\mathbf{\hat{P}_{dev}}$)
  \STATE Estimate the device position using the Levenberg--Marquardt Least Squares (L--MLS) Lateration method, with values $\mathbf{\hat{d}_{dev}}$ and  $\mathbf{\hat{P}_{dev}}$
  \RETURN $\hat{\hat{P}}_{dev}$
  \STATE \textbf{end Function}
  
  \STATE \textbf{ Share the second estimated device position ($\hat{\hat{P}}_{dev}$)}
  \STATE \textbf{Load devices position ($\mathbf{\hat{\hat{P}}_{dev}}$)}

  %%% Improve the accuracy of all estimated positioning
  
    %___________d\_btw\_Ps Function
  \STATE \textbf{Function} d\_btw\_Ps($\mathbf{\hat{\hat{P}}_{dev}}$, $\mathbf{\hat{P}_{dev}}$)
  \STATE Compute the relative distance between estimated device position $\mathbf{\hat{\hat{P}}_{dev}}$ and $\mathbf{\hat{P}_{dev}}$
  \RETURN $\mathbf{d_{\hat{\hat{P}}dev}}$ and $\mathbf{d_{\hat{P}dev}}$
  %\IF {$\mathbf{d_{\hat{\hat{P}}dev}}-\mathbf{d_{\hat{P}dev}}$}
  %\STATE Compute the relative 
  %\ELSE
  \STATE \textbf{end Function}
    %___________centroid\_Ps Function
  \STATE \textbf{Function} d\_btw\_Ps($\mathbf{\hat{\hat{P}}_{dev}}$, $\mathbf{\hat{P}_{dev}}$, $\mathbf{d_{\hat{\hat{P}}dev}}$)
  \STATE Compute the centroid of positions $\mathbf{\hat{\hat{P}}_{dev}}$ and $\mathbf{\hat{P}_{dev}}$, align both centroid and compute a new $\mathbf{\hat{\hat{\hat{P}}}_{dev}}$ based on the centroid and preserving the relation $\mathbf{d_{\hat{\hat{P}}dev}}$
  \RETURN $\mathbf{\hat{\hat{\hat{P}}}_{dev}}$
  \STATE \textbf{end Function}
 \end{algorithmic}
 \end{algorithm}


==> Algorithm/Algo_03.tex <==
\begin{algorithm}[!htb]
 \caption{Enhance of collaborative devices position}
 \label{alg:three}
 \begin{algorithmic}[1]
 \small
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
  \REQUIRE Estimated collaborative device positions $wt$ ($\hat{P}_{initdev}$ and $\hat{P}_{dev}$)
  \ENSURE Estimated position   $\hat{P}_{enhanced}$
  %%% Improve the accuracy of all estimated positioning
  \STATE \textbf{Call} d\_btw\_Ps($\hat{P}_{initdev}$, $\hat{P}_{dev}$)
  \STATE \textbf{Call} centroid\_Pos($\hat{P}_{initdev}$, $\hat{P}_{dev}$, $\mathbf{d_{dev}}$)
    %___________d\_btw\_Ps Function
  \STATE \textbf{Function} d\_btw\_Ps($\hat{P}_{initdev}$, $\hat{P}_{dev}$)
  \STATE Compute the relative distance between estimated device position $\hat{P}_{initdev}$, $\hat{P}_{dev}$
  \RETURN $\mathbf{d_{initdev}}$ and $\mathbf{d_{dev}}$
  \STATE \textbf{end Function}
    %___________centroid\_Ps Function
  \STATE \textbf{Function} centroid\_Pos($\hat{P}_{initdev}$, $\hat{P}_{dev}$, $\mathbf{d_{dev}}$)
  \STATE Compute the centroid of positions $\hat{P}_{initdev}$ and $\hat{P}_{dev}$, align both centroid and compute a new $\hat{P}_{enhanced}$ based on the centroid and preserving the relation $\mathbf{d_{dev}}$
  \RETURN $\hat{P}_{enhanced}$
  \STATE \textbf{end Function}
 \end{algorithmic}
 \end{algorithm}


==> Tables/NN_features.tex <==
\begin{table}[]
\caption{ANN features}
\label{tab_features}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccccc|c}
\toprule
\multirow{2}{*}{} & \multicolumn{6}{c|}{Input} & \multicolumn{1}{c}{Target} \\ 
\cline{2-8} 
 & \multicolumn{1}{c}{$RSS$} & \multicolumn{1}{c}{$X_T$} & \multicolumn{1}{c}{$Y_T$} & \multicolumn{1}{c}{$X_R$} & \multicolumn{1}{c}{$Y_R$} & \multicolumn{1}{c|}{$RSS_{1m}$} & \multicolumn{1}{c}{$d_{T-R}$} \\ 
 \midrule
ANN1 & * & * & * & * & * & * & * \\
ANN2 & * & * & * & * & * & - & * \\
ANN3 & * & - & - & * & * & * & * \\
ANN4 & * & * & * & - & - & * & * \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/beaconslist.tex <==
%\begin{table*}[ht]
\begin{table}[htbp]
\caption{Location of \ac{ble} anchors}%\acf{gt} position of \ac{ble} beacons and Smartphone device, and \ac{ble} beacons major and minor values}
\label{tab_beaconlist}
\centering
\tabcolsep 3pt
\aboverulesep = 0.15125mm%\belowrulesep = 0.241mm
\begin{tabular}{cccccccc}
\toprule
&
\multicolumn{4}{c}{Reference \ac{ble} beacons} \\ 
\cmidrule{2-5}
 No. & \multicolumn{1}{c}{x (\si{\meter})} & \multicolumn{1}{c}{y (\si{\meter})} & \multicolumn{1}{c}{TX Power (\si{\decibel})}& \multicolumn{1}{c}{TX Period (\si{\milli\second})} \\ 
 %\cline{2-5}\cline{7-8}
 % & \multicolumn{1}{c}{[m]} & \multicolumn{1}{c}{[m]} & \multicolumn{1}{c}{[dBm]}& \multicolumn{1}{c}{[ms]}&& \multicolumn{1}{c}{[m]} & \multicolumn{1}{c}{[m]}\\
%Name & function values & function value & &
%function values  \\ 
\midrule
1 & 0 &0 &-4 &250\\ 
%2 & 0 &2.61 &-4 &250 && 3.85&9.6\\ 
%3 & 0 &7.66 &-4 &250 && 1.15&6.1\\ 
2 & 0 &10.68 &-4 &250\\ 
%5 & 3.88 &3.54 &-4 &250 && 6.85&1.3\\ 
3 &  3.78 &6.51 &-4 &250\\ 
%7 &  3.87 &8.64 &-4 &250 && 9.25&9.6\\ 
%8 & 6.45 &2.13 &-4 &250 && 10.75&5.5\\ 
%9 & 6.66 &8.58 &-4 &250 && 11.65&1.3\\ 
4 & 6.68  &10.64 &-4 &250\\ 
5 & 9.2 &3.7 &-4 &250\\ 
%12 &  9.08 &5.95 &-4 &250 && 14.05&10\\ 
%13 &  9.18 &8.71 &-4 &250 && 12.55&6.1\\ 
%14 & 11.4  &3.6 &-4 &250 &&-- &--\\ 
%15 & 11.54 &7.18 &-4 &250 &&-- &--\\ 
%16 & 11.54 &10.65 &-4 &250 &&-- &--\\ 
%17 & 13.95 &4.34 &-4 &250 &&-- &--\\ 
6 &  14.2 &6.05 &-4 &250\\ 
%19 & 15.65 & 1.71 &-4 &250 &&-- &--\\ 
7 & 16.65 & 10.65 &-4 &250\\ 
\bottomrule
\end{tabular}
%\label{tab1}
\end{table}
